Can Image Models Imagine Time? ImageTime: A Novel Benchmark for Probing Visual World Modeling Through Spatiotemporal Consistency

Image generation models now produce high-quality static images, yet their ability to represent how a visual world changes over time remains poorly understood. Practical workflows such as storyboarding, step-by-step illustration, reference-guided editing, and video previsualization require models to preserve identities, objects, spatial relations, and causal order across multiple visual states. Existing evaluations largely measure single-image correctness, compositional alignment, or video quality, leaving open whether an image model can coherently imagine a temporally ordered process. We introduce ImageTime, a diagnostic benchmark that uses spatiotemporal consistency as a behavioral probe of visual world modeling in image generation. Given an action instruction, and optionally a reference image specifying the initial state, a model must generate one image containing four ordered key states: initial state, action onset, transition state, and final state. This four-keyframe protocol is more temporally demanding than single-image generation while avoiding the confounds of dense video dynamics. ImageTime organizes tasks with a progressive capability hierarchy and decomposes each scenario into stage-wise state predicates, cross-frame temporal constraints, and forbidden causal violations. GPT-5.5 scores all generated images under a structured VLM-as-judge protocol, producing interpretable capability scores, diagnostic subscores, and failure labels. Through multi-family benchmarking, ImageTime reveals where current image generation systems succeed, fail, and drift when asked to maintain coherent visual world states over time.

==> tables/generation_and_judging_config.tex <==
\begin{tabular}{@{}p{0.34\textwidth}p{0.58\textwidth}@{}}
\toprule
Model & Evaluation setting \\
\midrule
GPT Image 2 & Prompt-only ImageTime evaluation \\
Seedream 5.0 Lite & Prompt-only ImageTime evaluation \\
Nano Banana 2 & Prompt-only ImageTime evaluation \\
FLUX.2 Pro & Prompt-only ImageTime evaluation \\
Qwen-Image-2512 & Prompt-only ImageTime evaluation \\
Z-Image-Turbo & Prompt-only ImageTime evaluation \\
HunyuanImage-2.1 & Prompt-only ImageTime evaluation \\
SDXL & Prompt-only ImageTime evaluation \\
\bottomrule
\end{tabular}


==> tables/tree_level_prompt_only_scores.tex <==
\begin{tabular}{@{}lccccccc@{}}
\toprule
Model & L0 & L1 & L2 & L3 & L4 & L5 & L6 \\
\midrule
GPT Image 2 & 8.11 & 7.44 & 7.45 & 7.45 & 7.56 & 7.62 & 7.28 \\
Nano Banana 2 & 7.66 & 7.00 & 7.19 & 7.10 & 7.30 & 7.46 & 5.83 \\
Seedream 5.0 Lite & 7.55 & 6.71 & 6.67 & 6.62 & 6.82 & 6.73 & 6.73 \\
FLUX.2 Pro & 6.93 & 6.54 & 5.64 & 5.18 & 5.35 & 4.48 & 4.52 \\
Qwen-Image-2512 & 6.35 & 5.94 & 4.86 & 4.63 & 4.93 & 3.60 & 1.21 \\
Z-Image-Turbo & 6.35 & 6.48 & 4.96 & 4.55 & 4.55 & 3.29 & 1.44 \\
HunyuanImage-2.1 & 5.64 & 4.54 & 4.39 & 4.03 & 4.74 & 3.79 & 1.20 \\
SDXL & 2.99 & 2.13 & 1.21 & 1.37 & 1.26 & 0.49 & 0.61 \\
\bottomrule
\end{tabular}

